PAPyA: Performance Analysis of Large RDF Graphs Processing Made Easy

Prescriptive Performance Analysis (PPA) has shown to be more useful than traditional descriptive and diagnostic analyses for making sense of Big Data (BD) frameworks' performance. In practice, when processing large (RDF) graphs on top of relational BD systems, several design decisions emerge and cannot be decided automatically, e.g., the choice of the schema, the partitioning technique, and the storage formats. PPA, and in particular ranking functions, helps enable actionable insights on performance data, leading practitioners to an easier choice of the best way to deploy BD frameworks, especially for graph processing. However, the amount of experimental work required to implement PPA is still huge. In this paper, we present PAPyA 1, a library for implementing PPA that allows (1) preparing RDF graphs data for a processing pipeline over relational BD systems, (2) enables automatic ranking of the performance in a user-defined solution space of experimental dimensions; (3) allows user-defined flexible extensions in terms of systems to test and ranking methods. We showcase PAPyA on a set of experiments based on the SparkSQL framework. PAPyA simplifies the performance analytics of BD systems for processing large (RDF) graphs.We provide PAPyA as a public open-source library under an MIT license that will be a catalyst for designing new research prescriptive analytical techniques for BD applications.

==> Listings/AbstractExecutorLst.tex <==
% \begin{wrapfigure}[8]{r}{.65\textwidth}
% \vspace{-5pt}
% \begin{minipage}{0.65\textwidth}
% \scriptsize
% \begin{lstlisting}[language=python, frame=single, caption={Abstract Executor definition in \pap.},label={lst:abstractexecutor},captionpos=b]
% from abc import ABC, abstractmethod
% class Executor(ABC):
%   @abstractmethod
%   def run(self, experiment, runs, dataPath, logsPath):
%         pass
% \end{lstlisting}
% \end{minipage}
% \end{wrapfigure}

==> Listings/DPLst.tex <==
% \begin{wrapfigure}[20]{r}{.7\textwidth}
% \vspace{-15pt}
% \begin{minipage}{0.7\textwidth}
% \scriptsize
% \begin{lstlisting}[language=python, frame=single, caption={Part of schema generation in \pap Data Perperator.}, label={lst:dp},captionpos=b]
% from papya import DataPreperator
% class SparkDataPreparator(DataPreparator):
%   def __init__(self, RDFGraph g):
%   def generateST(self,g): # Step (1) in Figure 4
%     ST=map(lambda x: x.split("\t"), g)  
%   def getUniquePredicates(self,ST):# unique predicates list
%     runSQL("SELECT DISTINCT p from ST").toList()
%   def generateVP(self,ST): # Step (2) in Figure 4
%     uniquePredicates=getUniquePredicates(ST)
%     for p in uniquePredicates:
%      VPTable=runSQL(f"SELECT s, o From ST WHERE p={p}")
%   def generateWPT(self,ST):# Step (3) in Figure 4
%     uniquePredicates=getUniquePredicates(ST)
%       for p1  in uniquePredicates:
%        for p2 in uniquePredicates:
%         if(p1 != p2):
%           q = "SELECT s, Pr1.o, Pr2.o  
%                FROM (SELECT T1.s, T1.o 
%                      FROM ST T1 WHERE T1.o={p1}) Pr1
%                LEFT JOIN (SELECT T2.s, T2.o 
%                           FROM ST T2 WHERE T2.o={p2}) Pr2"
%           wptable=runSQL(q)
% \end{lstlisting}
% \end{minipage}
% \end{wrapfigure}

%  def generateExtVP(self,VP[],relType):# Step (4) in Figure 4
%     #getRelatedPredicates omitted due to space limits
%     relpreds = getRelatedPredicates(p1, relType)
%     for p2 in relpreds:
%         extVPcommand = ("SELECT t1.s, t1.o"
%           + "FROM {p1}  t1 "
%           + "LEFT SEMI JOIN  {p2} t2 ON ")
%         if (relType == "SS"){ #subject-to-subject joined
%           extVPcommand += "(t1.s=t2.s)"
%         } else if (relType == "OS"){#object-to-subject joined
%           extVPcommand += "(t1.o=t2.s)"
%         } else if (relType == "SO"){#subject-to-object joined
%           extVPcommand += "(t1.s=t2.o)"}
%         extVpTable = runSQL(extVPcommand)




%   def getRelatedPredicates(pred1, relType):
%  	RelPredsCmd = ("SELECT DISTINCT p FROM ST t1 
%  	LEFT SEMI JOIN "+ 
%         if (relType == "SS"){
%           RelPredsCmd += "(t1.s=t2.s)"
%         } else if (relType == "OS"){
%           RelPredsCmd += "(t1.s=t2.o)"
%         } else if (relType == "SO"){
%           RelPredsCmd += "(t1.o=t2.s)"}
%         runSQL(RelPredsCmd).toList()

==> Listings/EvaluationMetricsLst.tex <==
\begin{wrapfigure}[24]{r}{.7\textwidth}
\vspace{-15pt}
\begin{minipage}{0.7\textwidth}
\scriptsize
\begin{lstlisting}[language=python, frame=single, caption={Ranking criteria goodness as per Equations (2) and (3).} ,label={lst:ranker},captionpos=b]
from papya import Ranker
class BenchRanker(Ranker):
    def conformance(rankSet,q,k, h):
     criteria_table = rankSet.loc[bestOfSD(k)]
     criteria_table = criteria_table[criteria_table>h]
     count = criteria_table.count(axis=1)
     sum = count.sum(axis=0)
     conformance = 1-(sum/(k*q))
     return conformance
    #count number of (dis)agreements in 2 ranking sets. 
    def coherence(rankSet1, rankSet2):
        n = len(rankSet1)
        # both lists must be equal
        assert len(rankSet2) == n, 
        i, j = np.meshgrid(np.arange(n), np.arange(n))
        a = np.argsort(rankSet1)
        b = np.argsort(rankSet2)
        kendall_index = np.logical_or(np.logical_and(a[i] < 
        a[j], b[i] > b[j]), np.logical_and(a[i] > a[j], b[i] 
        < b[j])).sum()
        return kendall_index/(n*(n-1))
\end{lstlisting}
\end{minipage}
\end{wrapfigure}


==> Listings/MDRankingLst.tex <==
\begin{wrapfigure}[20]{r}{.6\textwidth}
\vspace{-15pt}
\begin{minipage}{0.63\textwidth}
\scriptsize
\begin{lstlisting}[language=python, frame=single, caption={MD-Ranking based on Pareto Fronts.},label={lst:mdrank},captionpos=b]
from papya import Rank
class MDRankPareto(Rank):
  # ds:dataset; dims:dimensions
  def eval(self, ds, dims): 
   # renkSet, function to get ranks of dataframe
   allDim = rankSet(ds,dims).reset_index().values
   inputPnt = np.array(rankSet(ds,dims)[:]).tolist()
   # pass nsga algorithm with prtQ function
   paretoPnts, dominatedPnts = nsga2(inputPnt, prtQ)
   # getConfs sort pareto solutions best->worst
   paretoQ = sort(paretoPnts, allDim)
   # pass nsga algorithm with prtAgg function
   paretoPnts, dominatedPnts = nsga2(inputPnt, prtAgg)
   paretoAgg = sort(paretoPnts, allDim)
   return paretoQ, paretoAgg
  def plot(self, paretoType):
   diagramPareto(paretoType)
\end{lstlisting}
\end{minipage}
\end{wrapfigure}

==> Listings/SDRankingLst.tex <==
\begin{wrapfigure}[17]{r}{.56\textwidth}
\vspace{-15pt}
\begin{minipage}{0.56\textwidth}
\scriptsize
\begin{lstlisting}[language=python, frame=single, caption={SD Ranking Function w.r.t Equation (1).}, label={lst:sdrank},captionpos=b]
from papya import Rank
class SDRank(Rank):
  #q is number of queries  
  def __init__(self, dimension, q): 
  def eval(self):
   d = len(self.dimension.index)
   rank_score = []
   for _, row in self.dimension.iterrows():
    for r in range(d):  
     s = s + (row[r+1]*(d-(r+1))/(self.q*(d-1)))
    rank_score.append(s)
   return rank_score
  def plot(self, rank_score):
   display(rank_score)
\end{lstlisting}
\end{minipage}
\end{wrapfigure}


==> OLDs/Top-3_confs_WatDiv.tex <==
%%%%%%%%%%%%%%Top-3 confs WatDiv%%%%%%%%%%%%%%%%%

% \begin{table}[t!]
% \footnotesize
% \centering
% \begin{tabular}{l||ccc|ccc|ccc}
% WatDiv         & \multicolumn{3}{c|}{100M}   & \multicolumn{3}{c|}{250M}   & \multicolumn{3}{c}{500M}    \\ \hline
% Rf             & a.ii.3  & a.i.3   & b.ii.2  & a.ii.3  & a.i.3   & b.iii.2 & a.ii.3  & a.i.3   & c.iii.2 \\ \hline
% Rp             & c.ii.2  & b.iii.3 & c.ii.1  & a.ii.1  & d.iii.3 & a.ii.2  & c.ii.2  & a.iii.2 & a.iii.4 \\ \hline
% Rs             & d.iii.4 & d.iii.1 & d.iii.3 & d.iii.4 & d.iii.3 & d.iii.2 & d.iii.2 & d.iii.4 & d.iii.1 \\ \hline
% Pareto$_{Agg}$ & c.ii.2  & d.iii.3 & b.ii.2  & d.iii.3 & c.i.4   & a.iii.4 & d.ii.2  & c.ii.3  & a.iii.4 \\ \hline
% Pareto$_{Q}$   & d.iii.2 & d.iii.3 & d.iii.4 & d.iii.2 & d.iii.3 & c.i.4   & d.ii.2  & d.iii.2 & d.i.2 
% \end{tabular}
% \caption{WatDiv best-performing (Top-3) configurations according to the SD and MD ranking criteria.}
% \label{tab:results_watdiv}
% \end{table}



==> OLDs/Top-5_confs_WatDiv_Full_ONLY.tex <==

%%%%%%%%%%%%%%Top-5 confs WatDiv Full ONLY %%%%%%%%%%%%%%%%%

% \begin{table}[t!]
% \scriptsize
% \centering
% \begin{tabular}{l|ccccc|ccccc|cccll}
% WatDiv       & \multicolumn{5}{c|}{100M}                      & \multicolumn{5}{c|}{250M}                       & \multicolumn{5}{c}{500M}                       \\ \hline
% Rf           & a.ii.3  & a.i.3   & b.ii.2  & a.iii.3 & b.i.2  & a.ii.3  & a.i.3   & b.iii.2 & c.iii.2 & a.iii.3 & a.ii.3  & a.i.3   & c.iii.2 & d.i.2   & d.ii.2 \\ \hline
% Rp           & c.ii.2  & b.iii.3 & c.ii.1  & b.iii.4 & a.ii.3 & a.ii.1  & d.iii.3 & a.ii.2  & c.i.4   & c.ii.1  & c.ii.2  & a.iii.2 & a.iii.4 & b.ii.2  & a.ii.1 \\ \hline
% Rs           & d.iii.4 & d.iii.1 & d.iii.3 & d.iii.2 & d.i.1  & d.iii.4 & d.iii.3 & d.iii.2 & d.iii.1 & c.i.1   & d.iii.2 & d.iii.4 & d.iii.1 & d.iii.3 & d.ii.2 \\ \hline
% Pareto$_{Agg}$ & c.ii.2 & d.iii.3 & b.ii.2 & a.ii.3 & d.iii.4 & d.iii.3 & c.i.4 & a.iii.4 & d.iii.4 & a.iii.3 & d.ii.2 & c.ii.3 & a.iii.4 & c.ii.4 & c.i.3 \\ \hline
% Pareto$_{Q}$ & d.iii.2 & d.iii.3 & d.iii.4 & c.ii.2  & c.i.2  & d.iii.2 & d.iii.3 & c.i.4   & d.i.2   & c.ii.2  & d.ii.2  & d.iii.2 & d.i.2   & c.i.3   & c.ii.3
% \end{tabular}

% \caption{WatDiv best-performing (\textit{Top-5}) configurations according to the SD and MD ranking criteria.}
% \label{tab:results_watdiv}
% \end{table}



==> OLDs/goodness_metrics_SP2B.tex <==
% \begin{table}[t!]
% \centering
% \begin{tabular}{l||c|c||c|c}
%               & \multicolumn{2}{c}{Coherence}                            & \multicolumn{2}{c}{Conformance} \\\hline
% Criteria  & distance & score & 100M                & 250M                \\\hline
% $R_f$          & $0.13$                       & $0.745$                   & 58\%                & 82\%                \\\hline
% $R_p$          & $0.18$                       & $0.67$                    & 61\%                & 70\%                \\\hline
% $R_s$          & $0.06$                       & $0.68$                    & 70\%                & 79\%                \\\hline
% $Pareto_{Agg}$ & $0.19$                       & $0.85$                    & 79\%                & 100\%               \\\hline
% $Pareto_{Q}$   & $0.24$                       & $0.80$                    & 85\%                & 100\%              
% \end{tabular}
% \caption{Ranking \textit{Coherence} \& \textit{Conformance} ($k$=3, $h$=17) across datasets.}
% \label{tab:goodness}
% \end{table}







% \begin{wraptable}[12]{r}{0.5\textwidth}
% \centering
% % \vspace{-5pt}
% \begin{tabular}{l||c|c||c|c}
%               & \multicolumn{2}{c}{Coherence}                            & \multicolumn{2}{c}{Conformance} \\\hline
% Criteria  & distance & score & 100M                & 250M                \\\hline
% $R_f$          & $0.13$                       & $0.745$                   & 58\%                & 82\%                \\\hline
% $R_p$          & $0.18$                       & $0.67$                    & 61\%                & 70\%                \\\hline
% $R_s$          & $0.06$                       & $0.68$                    & 70\%                & 79\%                \\\hline
% $Pareto_{Agg}$ & $0.19$                       & $0.85$                    & 79\%                & 88\%               \\\hline
% $Pareto_{Q}$   & $0.24$                       & $0.80$                    & 85\%                & 95\%              
% \end{tabular}
% \caption{Ranking \textit{Coherence} \& \textit{Conformance} ($k$=3, $h$=45) across datasets.}
% \label{tab:goodness}
% \end{wraptable}






%%%%%%%%%%% OLD Conformance and coherence SP2B%%%%%%%%%%%%%%%

% \begin{wraptable}[11]{r}{0.5\textwidth}
% \vspace{-20pt}
% \begin{tabular}{l|c||cc}
%                & Coherence & \multicolumn{2}{c}{Conformance}  \\ \hline
% Criteria       & 100M-250M & \multicolumn{1}{c|}{100M} & 250M \\ \hline
% $R_f$          & $0.17$    & \multicolumn{1}{c|}{58\%} & 82\% \\ \hline
% $R_p$          & $0.18$    & \multicolumn{1}{c|}{61\%} & 70\% \\ \hline
% $R_s$          & $0.07$    & \multicolumn{1}{c|}{70\%} & 79\% \\ \hline
% $Pareto_{Agg}$ & $0.19$    & \multicolumn{1}{c|}{79\%} & 88\% \\ \hline
% $Pareto_{Q}$   & $0.26$    & \multicolumn{1}{c|}{85\%} & 95\%
% \end{tabular}
% \caption{Ranking \textit{Coherence} \& \textit{Conformance} ($k$=3, $h$=45) across datasets.}
% \label{tab:goodness}
% \end{wraptable}


==> OLDs/old_intro.tex <==
% \begin{figure}[t!]
% \centering
% \includegraphics[width=1\linewidth]{Figures/BDPipeline.pdf}
% \caption{Big Data Pipeline}
% \label{fig:bdpipe}
% \vspace{-15 pt}
% \end{figure}



The growing popularity of Big Data (BD) frameworks for analytics is raising the awareness of their complexity. In particular, making sense of their performance appears to be one of the hardest tasks~\cite{ghazal2013bigbench}. If, on the one hand, BD frameworks enable scalable data analysis, they also pose significant challenges in identifying the experimental configurations that maximizes the performance~\cite{lu2019speedup}. To this extent, the database community started exploring techniques such as reinforcement learning to automate tuning of the systems' parameters (a.k.a. auto-tuneable knobs~\cite{van2021inquiry}), e.g., cache size and swap frequency. However, BD frameworks are substantially more complex than database systems due to their expressive APIs that allow the design of complex data pipelines~\cite{ragabieee21}. Such an issue aggravates even more in the case of analytical problems like querying large (RDF) graphs. Indeed, graph querying, by nature, imposes several design decisions that cannot be automatically tuned. For instance, deciding the relational schema to represent the graph still requires the intervention of a data engineer. With the size of graphs growing even further~\cite{sakr2021future}, the need for scalable yet interpretable methods for performance analysis becomes crucial.


In~\cite{ragab2021depth}, we highlight the severity of the problem by showing that the performance of BD systems for querying large (RDF) graphs may not be replicated. In particular, we showed that changing even just one experimental parameter, e.g., \textit{partitioning technique} or \textit{storage encoding}, invalidates existing optimizations in the relational representation of RDF data. 
%
We observe that issues do not lay in the way the investigations were conducted, but rather in the structure of the analysis, which is limited to \textit{descriptive} or at most \textit{diagnostic} observations of the system behavior. Such discussions leave much work for practitioners to transform observations into actionable insights.

Later in~\cite{ragabieee21}, we have introduced the concept of \textit{Bench-Ranking} as a means for enabling \textit{Prescriptive Performance Analysis} (PPA). The PPA is an alternative to descriptive/diagnostic discussions that aims to answer the question \textit{What should we do?}~\cite{lepenioti2020prescriptive}. In practice, \textit{Bench-Ranking} enables informed decision-making without neglecting the complexity of the performance analysis nor the performance trade-offs~\cite{ragabieee21}. 


Although, Bench-Ranking reduces the amount of time to gain PP, and deciding the best configurations of a BD system to execute a SPARQL query workload over a large RDF graphs. However, Implementing Bench-Ranking still demands huge engineering efforts and time to engineer the experiments. Indeed, in our direct experience, the most time-consuming phases for querying large RDF graphs divides between the \textit{data preparation} and \textit{results analytics}.


% Nevertheless, we remark that determining the best way to execute a SPARQL workload over a large RDF graph using a BD framework is still a \textit{time-consuming} task. 
%
% In our direct experience, only $30\%$ of the time is spent in executing the experiments, while the remainder divides between \textit{data preparation} task and \textit{results analytics}. 

To mitigate this problem, we present a library called \textit{\pap} (Prescriptive Analysis in Python Actions), which aims at 
(1) reducing the work and time required for data preparations and data loading; 
(2) reproducing existing experiments (according to users needs and convenience) for relational processing of SPARQL queries using SparkSQL. This will lead to reducing huge efforts for building analytical pipelines from scratch for new relational BD systems subject to experiments. Moreover, (3) automating the Bench-Ranking methods for prescriptive performance analysis described in~\cite{ragabieee21}. In practice, \pap facilitates navigating the complex solution space via packaging the functionality of different ranking functions as well as \textit{Multi-Optimization} (MO) techniques into interactive programmatic library interfaces. Last but not least, 
(4) checking the replicability of the relational BD systems' performance for querying large (RDF) graphs within a complex experimental solution space.

\vspace{3pt}

\noindent\textit{\textbf{Outline.}}
Section~\ref{sec:benchranking} briefly introduces the \textit{Bench-Ranking} framework~\cite{ragabieee21}.
Section~\ref{sec:lib_req_arch} presents the \pap requirements alongside its framework architecture.
Section~\ref{sec:bench_in_use} shows how to use \pap in practice, providing examples from existing experiments~\cite{ragab2021depth,ragabieee21}. 
Section~\ref{sec:relwork} discusses the related work and, finally, Section~\ref{sec:conclusion} concludes the paper and presents \pap's roadmap. 


==> SDFigs.tex <==
%this is an example for adding 6 small figures in two rows (three in each row). 

\begin{figure*}[t]
    \centering % <-- added
\medskip
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=0.65\linewidth]{Figures/SDFigs/schema_SBP.png}\quad
  \caption{\scriptsize SBP}
  \label{fig:4}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
     \includegraphics[width=0.65\linewidth]{Figures/SDFigs/schema_HP.png}\quad
 
 \caption{\scriptsize HP}
  \label{fig:5}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
     \includegraphics[width=0.65\linewidth]{Figures/SDFigs/schema_PBP.png}\quad
 \caption{\scriptsize PBP}
  \label{fig:6}
\end{subfigure}
%   \vspace{5pt}
\caption{Relational schemas ranking scores for the \textbf{500M} triples datasets (The higher the better).}
\label{fig:schemascores}
\end{figure*}

\begin{figure*}[h!]
\medskip
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=0.65\linewidth]{Figures/SDFigs/partitionin_ST.png}\quad
  \caption{\scriptsize ST}
  \label{fig:4}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
     \includegraphics[width=0.65\linewidth]{Figures/SDFigs/partitonin_VP.png}\quad

  \caption{\scriptsize VT}
  \label{fig:5}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
     \includegraphics[width=0.65\linewidth]{Figures/SDFigs/partiton_Pt.png}\quad
  \caption{\scriptsize PT}
  \label{fig:6}
\end{subfigure}

\caption{Partitioning techniques ranking for the \textbf{500M} triples datasets (The higher the better).}
\label{fig:partitioningscores}
\end{figure*}


\begin{figure*}[h!]
    \centering % <-- added
\medskip
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=0.65\linewidth]{Figures/SDFigs/storage_ST.png}\quad

  \caption{\scriptsize ST}
 

  \label{fig:4}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
     \includegraphics[width=0.65\linewidth]{Figures/SDFigs/storage_VP.png}\quad
     
  \caption{\scriptsize VT}
        

  \label{fig:5}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
     \includegraphics[width=0.65\linewidth]{Figures/SDFigs/storage_PT.png}\quad
      
  \caption{\scriptsize PT}

  \label{fig:6}
\end{subfigure}

\caption{Storage backends ranking scores for the \textbf{500M} triples datasets (The higher the better).}
\label{fig:backendscores}
% \vspace{-10pt}
\end{figure*}


==> Tables/QueryRuntimesTbl.tex <==
% % \vspace{-5pt}
% % \begin{table}[t]
% \scriptsize
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \backslashbox{Conf.}{Query} &
%   \multicolumn{1}{l|}{Q1} &
%   \multicolumn{1}{l|}{Q2} &
%   \multicolumn{1}{l|}{...} &
%   \multicolumn{1}{l|}{Q19} &
%   \multicolumn{1}{l|}{Q20} &
%   \multicolumn{1}{l|}{$R_{Q1}$}&  
%   \multicolumn{1}{l|}{$R_{Q2}$} &
%   \multicolumn{1}{l|}{...} &  
%   \multicolumn{1}{l|}{$R_{Q20}$}   \\ \hline
% a.i.1   & 63.85   & 50.91   & ... & 13.26   & 13.56  & $41^{th}$ & $41^{th}$ & ...& $40^{th}$ \\ \hline
% a.i.2   & 133.32   & 147.59  & ... & 45.88   & 46.84 & $44^{th}$ & $48^{th}$ & ...& $46^{th}$ \\ \hline
% ...     & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% b.iii.4   & 24.86   & 25.21   & ... & 6.10   & 7.56  & $11^{th}$ & $26^{th}$ & ...& $32^{th}$ \\ \hline
% ...     & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% % c.i.2 & 9.67  & 55.67   & ... & 17.93   & 7.61  \\ \hline
% \textbf{e.ii.4} & 205.28  & 162.34   & ... & 1.14   & 26.69 & $60^{th}$ & $60^{th}$ & ...& $42^{th}$  \\ \hline
% \end{tabular}
% \caption{Configuration rankings by query execution time $R_{Qx}$.}
% \label{tab:queryruntimes_rankings}
% % \end{table}
% \vspace{-5pt}
% \begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c||c|c|c|c|c|c|}
\hline
\backslashbox{Conf.}{Query} &
  \multicolumn{1}{l|}{Q1} &
  \multicolumn{1}{l|}{Q2} &
  \multicolumn{1}{l|}{...} &
  % \multicolumn{1}{l|}{Q19} &
  \multicolumn{1}{l||}{Q20} &
  \multicolumn{1}{l|}{Q1} &  
  \multicolumn{1}{l|}{Q2} &
  \multicolumn{1}{l|}{...} &  
  \multicolumn{1}{l|}{Q20}   \\ \hline
a.i.1   & 63.8   & 50.9   & ... &  13.5  & $41^{th}$ & $41^{th}$ & ...& $40^{th}$ \\ \hline
a.i.2   & 133.3   & 147.5  & ... & 46.8 & $44^{th}$ & $48^{th}$ & ...& $46^{th}$ \\ \hline
...     & ... & ... & ... & ... & ...  & ... & ... & ... \\ \hline
b.iii.4   & 24.8   & 25.2   & ...  & 7.5  & $11^{th}$ & $26^{th}$ & ...& $32^{th}$ \\ \hline
...     & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% c.i.2 & 9.67  & 55.67   & ... & 17.93   & 7.61  \\ \hline
\textbf{e.ii.4} & 205.2  & 162.3   & ...  & 26.6 & $60^{th}$ & $60^{th}$ & ...& $42^{th}$  \\ \hline
\end{tabular}
\caption{Configuration rankings by query execution time, e.g., (a.i.1) configuration is at $41^{th}$ rank in $Q1$.}
\label{tab:queryruntimes_rankings}
% \end{table}

==> Tables/RankScoresExample.tex <==
%%%%%%%%%%%%Ranking Scores Calculations Example%%%%%%%%%%%%%%%%%
% \begin{wraptable}[7]{r}{0.35\textwidth}
% \begin{table}[t]
% \end{table}
% \vspace{-25pt}
\centering
% \begin{center}
\scriptsize
\begin{tabular}{c|cccccc}
\hline
\textbf{Schema} & \textbf{1$^{st}$} & \textbf{2$^{nd}$} & \textbf{3$^{rd}$} &  \textbf{4$^{th}$}  &  \textbf{5$^{th}$}  & \textbf{R} \\ \hline

\cellcolor[HTML]{D9D9D9}\textbf{ExtVP} & 6 & 6 & 8 &  0 & 0& \cellcolor[HTML]{8C872E}0.73 \\ \hline

\cellcolor[HTML]{D9D9D9}\textbf{PT} & 6 & 6 & 5 &  2 & 1& \cellcolor[HTML]{8C872E}0.68 \\ \hline

\cellcolor[HTML]{D9D9D9}\textbf{WPT} & 7 & 3 & 0 &  0 & 10& \cellcolor[HTML]{A36F16}0.46 \\ \hline

\cellcolor[HTML]{D9D9D9}\textbf{ST} & 1 & 3 & 4 &  9 & 3& \cellcolor[HTML]{A36F16}0.38 \\ \hline

\cellcolor[HTML]{D9D9D9}\textbf{VP} & 0 & 2 & 3 & 9 & 6 & \cellcolor[HTML]{A36F1F}0.26 \\ \hline

\end{tabular}
\label{tab:formulaCalc}
\caption{Example of \textit{Rank Scores}.}
% \end{center}
% \end{wraptable}
% \end{table}


==> Tables/bestconfsSp2BNoPart.tex <==
% \begin{table}[t!]
% \centering
% \begin{tabular}{l||ccccc|ccccc}
% SP2Bench  & \multicolumn{5}{c}{100M}                        & \multicolumn{5}{|c}{250M}                        \\\hline
% Rf        & a.iii.3 & a.ii.3  & a.i.3  & b.ii.4   & d.ii.4   & a.iii.3 & a.ii.3  & b.ii.4  & b.i.4   & a.i.4   \\\hline
% % Rp        & a.ii.4  & a.ii.3  & a.ii.1  & b.ii.4  & b.ii.1  & b.ii.3  & a.ii.4  & b.ii.4  & a.ii.3  & d.ii.4  \\\hline
% Rs        & b.iii.1 & b.iii.2 & b.iii.4 & d.iii.2 & b.iii.3 & b.iii.4 & b.iii.3 & b.iii.1 & d.iii.2 & b.iii.2 \\\hline
% Pareto$_{Agg}$ & c.ii.2  & d.iii.1  & b.iii.2  & a.iii.3  & d.ii.1  & b.iii.4  & d.ii.2  & a.iii.3  & a.ii.3   & d.ii.4  \\\hline
% Pareto$_{Q}$   & e.ii.3  & e.ii.4 & e.i.3 & b.ii.4 & d.ii.4   & b.iii.4  & b.ii.3  & d.ii.4  & d.i.3   & d.i.4 
% \end{tabular}
% \vspace{5pt}
% \caption{SP2Bench best-performing confs. according to various ranking criteria.}
% \label{tab:results}
% \vspace{-20pt}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[t!]
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}c |c|c|c|c|l|lrrl|}
\hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}SP2Bench} &
  \multicolumn{1}{l|}{Rs} &
  \multicolumn{1}{l|}{Rf} &
  \multicolumn{1}{l|}{paretoQ} &
  \multicolumn{1}{l|}{paretoAgg} &
   &
  \multicolumn{4}{c|}{Evaluation Metrics} \\ \cline{1-5} \cline{7-10} 
\cellcolor[HTML]{FFFFFF} &
  b.2 &
  a.3 &
  b.4 &
  b.1 &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{c|}{Conformance} &
  \multicolumn{1}{c|}{Coherence} \\ \cline{2-5} \cline{8-10} 
\cellcolor[HTML]{FFFFFF} &
  b.1 &
  a.4 &
  b.1 &
  a.3 &
   &
  \multicolumn{1}{l|}{\multirow{-2}{*}{Criterion}} &
  \multicolumn{1}{l|}{100M} &
  \multicolumn{1}{l|}{250M} &
  100M-250M \\ \cline{2-5} \cline{7-10} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}100M} &
  c.2 &
  b.1 &
  b.2 &
  b.2 &
   &
  \multicolumn{1}{l|}{Rs} &
  \multicolumn{1}{r|}{81.82\%} &
  \multicolumn{1}{r|}{81.82\%} &
   \\ \cline{1-5} \cline{7-10} 
\cellcolor[HTML]{FFFFFF} &
  b.1 &
  a.3 &
  b.3 &
  b.4 &
   &
  \multicolumn{1}{l|}{Rf} &
  \multicolumn{1}{r|}{68.18\%} &
  \multicolumn{1}{r|}{95.45\%} &
   \\ \cline{2-5} \cline{7-10} 
\cellcolor[HTML]{FFFFFF} &
  b.3 &
  b.4 &
  b.4 &
  a.3 &
   &
  \multicolumn{1}{l|}{paretoQ} &
  \multicolumn{1}{r|}{77.27\%} &
  \multicolumn{1}{r|}{100.00\%} &
   \\ \cline{2-5} \cline{7-10} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}250M} &
  b.4 &
  b.3 &
  a.3 &
  b.1 &
  \multirow{-7}{*}{} &
  \multicolumn{1}{l|}{paretoAgg} &
  \multicolumn{1}{r|}{72.73\%} &
  \multicolumn{1}{r|}{95.00\%} &
   \\ \hline
\end{tabular}


\caption{Best-performing (Top-3) configurations, and ranking criteria evaluation metrics after excluding the partitioning dimension.}
\label{tab:sp2b_removing_part}

\end{table}

==> Tables/bestconfsWatDivNoPart.tex <==
\begin{table}[t!]
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}c |c|c|c|c|l|lrrl|}
\hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}WatDiv\_no\_Part} &
  \multicolumn{1}{l|}{$\mathcal{R}_{s}$} &
  \multicolumn{1}{l|}{$\mathcal{R}_{f}$} &
  \multicolumn{1}{l|}{Pareto$_{Q}$} &
  \multicolumn{1}{l|}{Pareto$_{Agg}$} &
   &
  \multicolumn{4}{c|}{WatDiv\_no\_Part Evaluation Metrics} \\ \cline{1-5} \cline{7-10} 
\cellcolor[HTML]{FFFFFF} &
  d.i.1 &
  a.i.3 &
  c.i.2 &
  c.i.2 &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{c|}{Conformance} &
  \multicolumn{1}{c|}{Coherence} \\ \cline{8-10} 
\cellcolor[HTML]{FFFFFF} &
  c.i.2 &
  b.i.2 &
  d.i.2 &
  b.i.2 &
   &
  \multicolumn{1}{l|}{\multirow{-2}{*}{Criterion}} &
  \multicolumn{1}{l|}{100M} &
  \multicolumn{1}{l|}{250M} &
  100M-250M \\ \cline{7-10} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}100M} &
  d.i.2 &
  e.i.4 &
  d.i.4 &
  d.i.1 &
   &
  \multicolumn{1}{l|}{$\mathcal{R}_{s}$} &
  \multicolumn{1}{r|}{97.50\%} &
  \multicolumn{1}{r|}{97.50\%} &
  \multicolumn{1}{r|}{0.11}   \\ \cline{1-5} \cline{7-10} 
\cellcolor[HTML]{FFFFFF} &
  c.i.1 &
  a.i.3 &
  d.i.2 &
  d.i.2 &
   &
  \multicolumn{1}{l|}{$\mathcal{R}_{f}$} &
  \multicolumn{1}{r|}{67.50\%} &
  \multicolumn{1}{r|}{30.00\%} &
\multicolumn{1}{r|}{ 0.17}  \\ \cline{7-10} 
\cellcolor[HTML]{FFFFFF} &
  d.i.2 &
  e.i.4 &
  c.i.4 &
  c.i.1 &
   &
  \multicolumn{1}{l|}{Pareto$_{Q}$} &
  \multicolumn{1}{r|}{95.00\%} &
  \multicolumn{1}{r|}{100.00\%} &
  \multicolumn{1}{r|}{0.11}   \\ \cline{7-10} 
  \multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}250M} &
  c.i.3 &
  d.i.2 &
  c.i.2 &
  e.i.4 &
  \multirow{-7}{*}{} &
  \multicolumn{1}{l|}{Pareto$_{Agg}$} &
  \multicolumn{1}{r|}{92.50\%} &
  \multicolumn{1}{r|}{97.50\%} &
 \multicolumn{1}{r|}{0.19}  \\ \hline
\end{tabular}

\caption{ Best-performing (Top-3) configurations, and ranking criteria evaluation metrics after \textbf{excluding the partitioning} dimension.}
\label{tab:sp2b_removing_part}

\end{table}

==> Tables/evaluation_metrics_WatDiv_Full.tex <==
%%%%%%%%%%%Conformance and Coherence for WatDiv%%%%%%%%%%%%%
\begin{table}[t!]
\scriptsize
\begin{tabular}{l|ccc|ccc|}
 &
  \multicolumn{3}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Conformance}} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Coherence}} \\ \cline{2-7} 
  \multirow{-2}{*}{} &
  \multicolumn{1}{l|}{\textbf{100M}} &
  \multicolumn{1}{l|}{\textbf{250M}} &
  \multicolumn{1}{l|}{\textbf{500M}} &
  \multicolumn{1}{l|}{\textbf{100M-250M}} &
  \multicolumn{1}{l|}{\textbf{100M-500M}} &
  \multicolumn{1}{l|}{\textbf{250M-500M}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{$\mathcal{R}_s$} &
  \multicolumn{1}{c|}{96.0\%} &
  \multicolumn{1}{c|}{94.0\%} &
  93.0\% &
  \multicolumn{1}{c|}{0.10} &
  \multicolumn{1}{c|}{0.13} &
  0.07 \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{$\mathcal{R}_p$} &
  \multicolumn{1}{c|}{73.0\%} &
  \multicolumn{1}{c|}{39.0\%} &
  36.0\% &
  \multicolumn{1}{c|}{0.09} &
  \multicolumn{1}{c|}{0.28} &
  0.17 \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{$\mathcal{R}_f$} &
  \multicolumn{1}{c|}{64.0\%} &
  \multicolumn{1}{c|}{32.0\%} &
  43.0\% &
  \multicolumn{1}{c|}{0.14} &
  \multicolumn{1}{c|}{0.25} &
  0.15 \\ \hline
\cellcolor[HTML]{EFEFEF} pareto$_{Q}$ &
  \multicolumn{1}{c|}{92.0\%} &
  \multicolumn{1}{c|}{98.0\%} &
  98.0\% &
  \multicolumn{1}{c|}{0.10} &
  \multicolumn{1}{c|}{0.15} &
  0.07 \\ \hline
\cellcolor[HTML]{EFEFEF} pareto$_{Agg}$ &
  \multicolumn{1}{c|}{87.0\%} &
  \multicolumn{1}{c|}{71.0\%} &
  76.0\% &
  \multicolumn{1}{c|}{0.17} &
  \multicolumn{1}{c|}{0.24} &
  0.15 \\ \hline

\cellcolor[HTML]{EFEFEF}\textbf{$\mathcal{R}_{ta}$} &
  \multicolumn{1}{c|}{89.0\%} &
  \multicolumn{1}{c|}{84.0\%} &
  76.0\% &
  \multicolumn{1}{c|}{0.15} &
  \multicolumn{1}{c|}{0.22} &
  0.13 \\ \hline
  
\end{tabular}
\caption{Ranking \textit{Coherence} (Kendal distance, the lower the better) \& \textit{Conformance} ($k$=5, $h$=28) across \textit{WatDiv} datasets.}
\label{tab:eval_metrics_watDiv_full}
\end{table}

==> Tables/topconfsSP2B.tex <==
\begin{table}[t!]
\footnotesize
\centering
\begin{tabular}{l||ccccc|ccccc}
SP2Bench  & \multicolumn{5}{c}{100M}                        & \multicolumn{5}{|c}{250M}                        \\\hline
Rf        & a.iii.3 & a.ii.3  & a.i.3  & b.ii.4   & d.ii.4   & a.iii.3 & a.ii.3  & b.ii.4  & b.i.4   & a.i.4   \\\hline
Rp        & a.ii.4  & a.ii.3  & a.ii.1  & b.ii.4  & b.ii.1  & b.ii.3  & a.ii.4  & b.ii.4  & a.ii.3  & d.ii.4  \\\hline
Rs        & b.iii.1 & b.iii.2 & b.iii.4 & d.iii.2 & b.iii.3 & b.iii.4 & b.iii.3 & b.iii.1 & d.iii.2 & b.iii.2 \\\hline
Pareto$_{Agg}$ & c.ii.2  & d.iii.1  & b.iii.2  & a.iii.3  & d.ii.1  & b.iii.4  & d.ii.2  & a.iii.3  & a.ii.3   & d.ii.4  \\\hline
Pareto$_{Q}$   & e.ii.3  & e.ii.4 & e.i.3 & b.ii.4 & d.ii.4   & b.iii.4  & b.ii.3  & d.ii.4  & d.i.3   & d.i.4 
\end{tabular}
\vspace{5pt}
\caption{SP2Bench best-performing confs. according to various ranking criteria.}
\label{tab:results_sp2b}
% \vspace{-20pt}
\end{table}

==> Tables/topconfsWatDiv_Full_Mini.tex <==
\begin{table}[]
\scriptsize
\centering
\begin{tabular}{l|ccccc|ccccc|cccll}
\textbf{Full-WatDiv} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{100M}} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{250M}} & \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{500M}} \\ \hline

Rf & a.ii.3 & a.i.3 & b.ii.2 & a.iii.3 & b.i.2 & a.ii.3 & a.i.3 & b.iii.2 & c.iii.2 & a.iii.3 & a.ii.3 & a.i.3 & c.iii.2 & d.i.2 & d.ii.2 \\ \hline

Rp & c.ii.2 & b.iii.3 & c.ii.1 & b.iii.4 & a.ii.3 & a.ii.1 & d.iii.3 & a.ii.2 & c.i.4 & c.ii.1 & c.ii.2 & a.iii.2 & a.iii.4 & b.ii.2 & a.ii.1 \\ \hline

Rs & d.iii.4 & d.iii.1 & d.iii.3 & d.iii.2 & d.i.1 & d.iii.4 & d.iii.3 & d.iii.2 & d.iii.1 & c.i.1 & d.iii.2 & d.iii.4 & d.iii.1 & d.iii.3 & d.ii.2 \\ \hline

Pareto$_{Q}$ & d.iii.2 & d.iii.3 & d.iii.4 & c.ii.2 & c.i.2 & d.iii.2 & d.iii.3 & c.i.4 & d.i.2 & c.ii.2 & d.ii.2 & d.iii.2 & d.i.2 & c.i.3 & c.ii.3 \\ \hline

Pareto$_{Agg}$ & c.ii.2 & d.iii.3 & b.ii.2 & a.ii.3 & d.iii.4 & d.iii.3 & c.i.4 & a.iii.4 & d.iii.4 & a.iii.3 & d.ii.2 & c.ii.3 & a.iii.4 & c.ii.4 & c.i.3 \\ \hline

$R_{ta}$ & c.ii.2 & d.iii.3 & b.ii.2 & d.iii.2  & a.ii.3 & d.iii.3 & c.i.4 & a.iii.4  & c.ii.1 & d.iii.4 & c.ii.3 & d.ii.2 & a.iii.4  & c.ii.4 & c.i.3 \\ 
\hline \hline 


\textbf{Mini-WatDiv} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{100M}} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{250M}} & \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{500M}} \\ \cline{2-16} 
Rf & a.ii.3 & b.ii.2 & a.i.3 & b.i.2 & c.ii.2 & a.ii.3 & a.i.3 & c.i.4 & b.ii.2 & b.i.2 & a.ii.3 & a.i.3 & c.i.3 & c.ii.3 & b.ii.2 \\ \hline
Rp & a.ii.3 & a.ii.4 & a.ii.2 & c.ii.2 & b.ii.2 & a.ii.3 & a.ii.4 & a.ii.2 & b.ii.2 & c.i.4 & a.ii.3 & a.ii.4 & a.ii.2 & c.ii.2 & b.ii.2 \\ \hline
Rs & c.i.4 & c.ii.2 & c.i.3 & c.ii.4 & c.i.2 & c.i.4 & c.i.3 & c.i.2 & c.ii.4 & c.ii.2 & c.ii.4 & c.i.4 & c.i.3 & c.ii.3 & c.ii.2 \\ \hline

Pareto$_{Q}$ & c.ii.2 & c.i.2 & b.ii.2 & b.i.2 & c.i.4 & c.i.4 & c.ii.2 & c.i.2 & c.i.3 & c.ii.4 & c.ii.3 & c.ii.4 & c.i.3 & c.i.4 & c.ii.2 \\ \hline

Pareto$_{Agg}$ & a.ii.3 & c.ii.2 & b.ii.2 & c.i.4 & - & c.i.4 & b.ii.2 & a.ii.3 & - & - & b.ii.2 & c.ii.3 & c.ii.4 & a.ii.3 & c.ii.2 \\ \hline

$R_{ta}$ & a.ii.3 & c.ii.2 & b.ii.2 & a.ii.4 & b.i.2 & c.i.4 & b.ii.2 & a.ii.3 & c.ii.2 & c.ii.3 & b.ii.2 & c.ii.3 & c.ii.4 & a.ii.3 & c.ii.2 \\ \hline 
\end{tabular}

\caption{WatDiv best-performing (\textit{Top-5}) configurations according to the SD and MD ranking criteria.}
\label{tab:results_watdiv}
\end{table}

